Non-Uniform $k$-Center and Greedy Clustering

In the Non-Uniform $k$-Center problem, a generalization of the famous $k$-center clustering problem, we want to cover the given set of points in a metric space by finding a placement of balls with specified radii. In $t$-NU$k$C Problem, we assume that the number of distinct radii is equal to $t$, and we are allowed to use $k_i$ balls of radius $r_i$, for $1 \le i \le t$. This problem was introduced by Chakrabarty et al. [ACM Trans. Alg. 16(4):46:1-46:19], who showed that a constant approximation for $t$-NU$k$C is not possible if $t$ is unbounded. On the other hand, they gave a bicriteria approximation that violates the number of allowed balls as well as the given radii by a constant factor. They also conjectured that a constant approximation for $t$-NU$k$C should be possible if $t$ is a fixed constant. Since then, there has been steady progress towards resolving this conjecture -- currently, a constant approximation for $3$-NU$k$C is known via the results of Chakrabarty and Negahbani [IPCO 2021], and Jia et al. [To appear in SOSA 2022]. We push the horizon by giving an $O(1)$-approximation for the Non-Uniform $k$-Center for $4$ distinct types of radii. Our result is obtained via a novel combination of tools and techniques from the $k$-center literature, which also demonstrates that the different generalizations of $k$-center involving non-uniform radii, and multiple coverage constraints (i.e., colorful $k$-center), are closely interlinked with each other. We hope that our ideas will contribute towards a deeper understanding of the $t$-NU$k$C problem, eventually bringing us closer to the resolution of the CGK conjecture.

==> prelims-robust.tex <==
\section{Preliminaries}

\subsection{Problem Definitions}

In the following, we set up the basic notation and define the problems we will consider in the paper. We consider a finite metric space $(X, d)$, where $X$ is a finite set of (usually $n$) points, and $d$ is a distance function satisfying triangle inequality. If $Y$ is a subset of $X$, then by slightly abusing the notation, we use $(Y, d)$ to denote the metric space where the distance function $d$ is restricted to the points of $Y$. Let $p \in X$, $Y \subseteq X$, and $r \ge 0$. Then, we use $d(p, Y) \coloneqq \min_{y \in Y} d(p, y)$, and denote by $B(p, r)$ the \emph{ball} of radius $r$ centered at $p$, i.e., $B(p, r) \coloneqq \{ q \in X : d(p, q) \le r \}$. We say that a ball $B(p, r)$ \emph{covers} a point $q$ iff $q \in B(p, r)$; a set of balls $\B$ (resp.\ a tuple of sets of balls $(\B_1, \B_2, \ldots, \B_t)$) covers $q$ if there exists a ball in $\B$ that covers $q$ (resp.\ $\bigcup_{1 \le i \le t} \B_i$ that covers $q$). Analogously, a set of points $Y \subseteq X$ is covered iff every point in $Y$ is covered. For a function $f: S \to \real^+$ or $f: S \to \natural$, and $R \subseteq S$, we define $f(R) \coloneqq \sum_{r \in R} f(r)$.

\begin{definition}[Decision Version of $t$-\nukc]
	\ \\The input is an instance $\I = ((X, d), (k_1, k_2, \ldots, k_t), (r_1, r_2, \ldots, r_t))$, where $r_1 \ge r_2 \ge \ldots r_t \geq 0$, and each $k_i$ is a non-negative integer. The goal is to determine whether there exists a solution $(\B_1, \B_2, \ldots, \B_t)$, where for each $1 \le i \le t$, $\B_i$ is a set with at most $k_i$ balls of radius $r_i$, that covers the entire set of points $X$. Such a solution is called a \emph{feasible solution}, and if the instance $\I$ has a feasible solution, then $\I$ is said to be \emph{feasible}.
	\\An algorithm is said to be an $\alpha$-approximation algorithm (with $\alpha \ge 1$), if given a feasible instance $\I$, it returns a solution $(\B_1, \B_2, \ldots, \B_t)$, where for each $1 \le i \le t$, $\B_i$ is a collection of at most $k_i$ balls of radius $\alpha r_i$, such that the solution covers $X$. 
\end{definition} 
Next, we define the robust version of $t$-\nukc.
\begin{definition}[Decision Version of Robust $t$-\nukc]
	\ \\The input is an instance $\I = ((X, d), (\omega, m), (k_1, k_2, \ldots, k_t), (r_1, r_2, \ldots, r_t))$. The setup is the same as in $t$-\nukc, except for the following: $\omega: X \to \integer^+$ is a weight function, and $1 \le m \le w(X)$ is a parameter. The goal is to determine whether there exists a feasible solution, i.e., $(\B_1, \B_2, \ldots, \B_t)$ of appropriate sizes and radii (as defined above), such that the total weight of the points covered is at least $m$. An $\alpha$-approximate solution covers points of weight at least $m$ while using at most $k_i$ balls of radius $\alpha r_i$ for each $1 \le i \le t$.
\end{definition}
We will frequently consider the \emph{unweighted} version of Robust $t$-\nukc, i.e., where the weight of every point in $X$ is unit. Let $\mathbbm{1}$ denote this unit weight function. Now we define the Colorful $t$-\nukc problem, which generalizes Robust $t$-\nukc.
\begin{definition}[Decision Version of Colorful $t$-\nukc]
	\ \\The input is an instance $\I= ((X, d), (w_r, w_b, m_r, m_b) , (k_1, k_2, \ldots, k_t), (r_1, r_2, \ldots, r_t))$. The setup is similar as in Robust $t$-\nukc, except that we have \emph{two} weight functions $w_r, w_b: X \to \real^+$ (corresponding to \emph{red} and \emph{blue} weight respectively). A feasible solution covers a set of points with red weight at least $m_r$, and blue weight at least $m_b$. The notion of approximation is the same as above.
\end{definition}
We note that the preceding definition naturally extends to an arbitrary number $\chi \ge 2$ of colors (i.e., $\chi$ different weight functions over $X$). However, we will not need that level of generality in this paper. 

\subsection{From $(t+1)$-NUkC to $t$-Robust-NUkC} \label{subsec:t-nukc-to-robust}

In this section, we show an approximate equivalence of $t+1$-NUkC and unweighted $t$-Robust-NUkC. In particular, we show the following lemma.
\begin{lemma}\label{lem:tplus1-to-t}\ 
	\begin{enumerate}
		\item Suppose there exists an $\alpha$-approximation algorithm for $t+1$-NUkC. Then, there exists an $\alpha$-approximation algorithm for unweighted $t$-Robust NUkC.
		\item Suppose there exists a $\beta$-approximation algorithm for unweighted $t$-Robust-NUkC. Then there exists a $3\beta+2$-approximation algorithm for $t+1$-NUkC.
	\end{enumerate}
\end{lemma}
\begin{proof}
Note that the first claim is trivial, since an instance of $t$-Robust-NUkC is a special case of NUkC, as follows. Let $\I = ((X, d), (\mathbbm{1}, m), (r_1, r_2, \ldots, r_t), (k_1, k_2, \ldots, k_t))$ be an instance of unweighted $t$-Robust-NUkC, where $m$ is the coverage requirement. Then, observe that it is equivalent to the instance $\I' = ((X, d), (r_1, r_2, \ldots, r_t, 0), (k_1, k_2, \ldots, k_t, n-m))$ of $t+1$-NUkC. An $\alpha$-approximate solution to $\I'$ immediately gives an $\alpha$-approximate solution to $\I$. We now proceed to the second claim.

Consider an instance $\I = ((X, d), (r_1, r_2, \ldots, r_t, r_{t+1}), (k_1, k_2, \ldots, k_t, k_{t+1}))$ of $(t+1)$-NUkC. Note that we have to cover all points of $X$ in the instance $\I$. First, we compute a $2r_{t+1}$-net $Y$ of $X$. That is compute $Y \subseteq X$ with the following properties: (i) $d(u, v) > 2r_{t+1}$ for any $u, v \in Y$, and (ii) for any $u \in X \setminus Y$, there exists a $v \in Y$ such that $d(u, v) \le 2r_{t+1}$. Let $\varphi: X \to Y$ be a mapping that assigns every point in $X$ to its nearest point in $Y$ (breaking ties arbitrarily). Our reduction constructs the instance $\I' = ((Y, d), (\mathbbm{1}, |Y|-k_{t+1}), (k_1, k_2, \ldots, k_t), (r'_1, r'_2, \ldots, r'_t))$ of $t$-Robust-NUkC with at most $k_{t+1}$ outliers, where $r'_i = r_i + 2r_t$ for $1 \le i \le t$.

We now argue that if $\I$ is feasible, then so is $\I'$.
Fix a solution $(\B_i)_{i \in [t+1]}$ for the original instance $\I$, where $\B_i$ is a set of at most $k_i$ balls of radius $r_i$. Let $Y' \subseteq Y$ be the set of points in $Y$ covered by $(\B_i)_{i \in [t]}$, the balls of the $t$ largest radii types. For each ball $B(c_i, r_i) \in \B_i$, we add $B(\varphi(c_i), r'_i)$ to obtain the set $\B'_i$ of balls; recall $r'_i = r_i + 2r_t$. Note that the resulting solution $(\B'_i)_{i \in [t]}$ covers the set of points $Y'$. Now, let $Y'' = Y \setminus Y'$ be the set of points covered by $\B_{t+1}$, the balls of radius $r_{t+1}$. The distance between any two points of $Y$, and thus $Y''$, is greater than $2r_{t+1}$. Therefore, a ball of radius radius $r_{t+1}$ covers at most one point of $Y''$, which implies that $|Y''| \le |\B_{t+1}| \le k_{t+1}$. Thus $(\B'_i)_{i \in [t]}$ is a feasible solution for instance $\I'$, with the points in $Y''$ being the set of outliers of size at most $k_{t+1}$.

We now argue that from a $\beta$-approximate solution to $\I'$, we can efficiently construct a $(3\beta + 2)$-approximate solution to $\I$. Fix a solution $(\B'_i)_{i \in [t]}$ for the instance $\I'$ that covers at least $|Y|-k_{t+1}$ points of $Y$, where $\B'_i$ consists of $k_i$ balls of radius $\beta r'_{i}$, for $1 \le i \le t$. To obtain a solution for the original instance $\I$, we proceed as follows. We expand the radius of every ball in $\B'_i$ by an additive factor of $2r_{t+1}$ to obtain $\B_i$. Note that the resulting radius for each ball in $\B_i$ is $\beta r_i + 2\beta r_{t+1} + 2r_{t+1} \le (3\beta+2) \cdot r_{i}$. Note that if a ball in solution $(\B'_i)_{i \in [t]}$ covers $y \in Y$, then the additively expanded version of the ball covers every point $x \in \varphi^{-1}(y)$. For every outlier point $y \in Y$ not covered by $(\B'_i)_{i \in [t]}$, we add a ball of radius $2r_{t+1}$ centered at $y$ to $\B_{t+1}$; this ball covers all points $x \in \varphi^{-1}(y)$. As the number of outliers is at most $k_{t+1}$, we have $|\B_{t+1}| \leq k_{t+1}$. The resulting solution $(\B_i)_{i \in [t+1]}$ covers all the points of $X$, and has approximation guarantee $3\beta+2$.
\end{proof}

